Opening the AI black box: program synthesis via mechanistic interpretability

We present MIPS, a novel method for program synthesis based on automated mechanistic interpretability of neural networks trained to perform the desired task, auto-distilling the learned algorithm into Python code. We test MIPS on a benchmark of 62 algorithmic tasks that can be learned by an RNN and find it highly complementary to GPT-4: MIPS solves 32 of them, including 13 that are not solved by GPT-4 (which also solves 30). MIPS uses an integer autoencoder to convert the RNN into a finite state machine, then applies Boolean or integer symbolic regression to capture the learned algorithm. As opposed to large language models, this program synthesis technique makes no use of (and is therefore not limited by) human training data such as algorithms and code from GitHub. We discuss opportunities and challenges for scaling up this approach to make machine-learned models more interpretable and trustworthy.

==> programs/control_program_input.tex <==
\newcommand{\docnr}{\getdata[1]\mydata}
\newcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[2]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[3]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[4]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[5]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[6]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[7]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[8]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[9]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[10]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[11]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[12]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[13]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[14]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[15]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[16]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[17]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[18]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[19]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[20]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[21]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[22]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[23]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[24]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[25]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[26]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[27]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\end{minipage}

\renewcommand{\docnr}{\getdata[28]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[29]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[30]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[31]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}

\renewcommand{\docnr}{\getdata[32]\mydata}
\renewcommand{\tocfile}{}
\begin{minipage}{\columnwidth}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}
\end{minipage}
\begin{comment}

\renewcommand{\docnr}{\getdata[33]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}


\renewcommand{\docnr}{\getdata[34]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[35]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[36]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[37]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[38]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[39]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[40]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[41]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[42]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[43]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[44]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[45]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[46]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[47]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[48]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[49]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[50]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[51]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[52]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[53]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[54]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[55]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[56]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[57]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[58]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[59]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[60]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[61]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[62]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[63]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[64]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[65]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[66]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[67]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[68]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[69]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[70]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[71]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[72]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[73]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[74]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[75]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[76]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[77]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[78]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[79]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\renewcommand{\docnr}{\getdata[80]\mydata}
\docnr
\makeatletter
\edef\docnr@wosp{\docnr\space}
\renewcommand{\tocfile}{}
\edef\tocfile{./programs/\expandafter\zap@space\docnr@wosp\@empty.txt}
\makeatother
\lstinputlisting[language=Python]{\tocfile}

\end{comment}
